MoTIF: Learning Motion Trajectories with Local Implicit Neural Functions for Continuous Space-Time Video Super-Resolution

This work addresses continuous space-time video super-resolution (C-STVSR) that aims to up-scale an input video both spatially and temporally by any scaling factors. One key challenge of C-STVSR is to propagate information temporally among the input video frames. To this end, we introduce a space-time local implicit neural function. It has the striking feature of learning forward motion for a continuum of pixels. We motivate the use of forward motion from the perspective of learning individual motion trajectories, as opposed to learning a mixture of motion trajectories with backward motion. To ease motion interpolation, we encode sparsely sampled forward motion extracted from the input video as the contextual input. Along with a reliability-aware splatting and decoding scheme, our framework, termed MoTIF, achieves the state-of-the-art performance on C-STVSR. The source code of MoTIF is available at https://github.com/sichun233746/MoTIF.

==> Chapter/3_proposed_method/Frame_Reconsruction.tex <==
\subsection{Frame Reconstruction}
\label{subsec:frame_reconstruction}
To reconstruct the high-resolution target frame $I_t^H$, we use multi-layer perceptrons as our pixel-wise decoder, which can adapt to different resolution. As shown in Fig. \ref{fig:overview}, the decoder takes several inputs: the nearest up-sampled intermediate feature map $F_{(0,1)}^H$ to serve as a initial prediction; the forward warped feature map $F_{t}^H$ that aggregate information temporally; the reliability map $\hat{Z}_{t}^H$ to indicate the reliable region of $F_{t}^H$; the time $t$ to provide time information. Note that introducing the reliability map $\hat{Z}_{t}^H$ to decoder helps the decoder rely more on the forward warped feature map $F_{t}^H$ or the initial prediction $F_{t}^L$.


% [origin] To reconstruct the high-resolution target frame $I_t^H$ at the moment $t$, we use multi-layer perceptrons as our pixel-wise decoder, which can adapt to different resolution. As shown in Fig. \ref{fig:overview}, the decoder takes several inputs: the nearest up-sampled intermediate feature map $F_{(0,1)}^H$ to serve as a residual; the forward warped feature map $F_{t}^H$ to aggregate information temporally; the reliability map $\hat{Z}_{t}^H$ to indicate the reliable region of $F_{t}^H$; the time $t$ to provide time information.

% [origin] To optimize our network, we use a reconstruction loss and a flow regularization loss which can be formulated as
% \begin{equation}
% L = L_{rec} + \beta \cdot L_{flow}
% \end{equation}

% [origin] The reconstruction loss models how similar to the ground truth frames our predicted frames are, which can be written as
% \begin{equation}
% L_{rec} = 
% L_{char}(\hat{I}_t^H,I_t^H)
% \end{equation}
% where $L_{char}(\hat{I},I)=\sqrt{\|{\hat{I}-I}\|^2+\epsilon^2}$ is the Charbonnier loss. The $\epsilon$ is set to $10^{-3}$ in our experiments.

% [origin] The flow regularization loss regularizes every predicted motion should be as close to the ground truth flow $\mathcal{M}_{ref}^H$ generated by off-the-shelf optical flow estimator, which makes our predicted motions explicit and explainable. The flow regularization loss can be expressed as
% \begin{equation}
% L_{flow} = 
% L_{char}(\hat{M}_{0\xrightarrow[]{}t}^H,{M}_{0\xrightarrow[]{}t}^H)+
% L_{char}(\hat{M}_{1\xrightarrow[]{}t}^H,{M}_{1\xrightarrow[]{}t}^H)
% \end{equation}

==> Chapter/3_proposed_method/Multi_Frame_Extension.tex <==
\textcolor{blue}{
\subsection{Generalization to More Reference Frames}
\label{subsec:multi_frame_extension}
To generate the high-resolution video frame $\hat{I}_t^H$, our scheme can be generalized to accommodate more than two reference frames. First, the generation of the motion latents can benefit from having more reference frames. For example, the motion latent $T_0^L$ may encode jointly information from multiple pairs of the forward flow map and its reliability map, $M_{0 \rightarrow i}^L,Z_{0 \rightarrow i}^L$, with $i$ referring to the reference frames except $I_{0}^L$. Conceptually, having access to a number of reference frames, e.g.~$N$ frames, allows us to take more forward motion samples $\{M_{0 \rightarrow i}^L\}_{i=1}^{N-1}$, which help construct accurate motion trajectories. Likewise, it is advantageous to aggregate more reference features $\{F_i^H\}_{i=0}^{N-1}$ in synthesizing $F_t^H,Z_t^H$. To this end, the summation/maximum operation over $i$ in Eqs.~\eqref{eq:warp_F} and~\eqref{eq:warp_Z} may
involve all the reference frames. }


%Real-world video sequences are always consecutive.
%From Section~\ref{subsec:method_overview} to \ref{subsec:training_objectives}, we focus on taking two adjacent video frames $I^L_0$ and $I^L_1$ as input to predict a high-resolution image $\hat{I}^H_t$ at time instance $t$. However, our \textcolor{red}{[OurModelName]} can be generalized to utilize any number of reference frames in two different ways: (1) Adopt additional reference frames (e.g. $I^L_{-1}, I^L_2$) to predict more precise motion trajectories. Since the forward motions between each reference frame can be easily obtained by the motion estimator, we use these forward motions (e.g. $M^L_{0\xrightarrow[]{}-1}, M^L_{0\xrightarrow[]{}2}$) as extra observations to model a more precise motion trajectory. We provide an experiment about this part in Section~\ref{sec:ablation}. (2) Warp extra reference frames (e.g. $I^L_{-1}, I^L_2$) to generate better high-resolution images. Except for forward motion trajectory modeling, all components of our framework can take arbitrary number of input frames using the same model. We conduct experiment about taking four reference frames for F-STVSR and demonstrate comparable performance to the state-of-the-arts in the supplementary document.

==> Chapter/4_experiment/Forward_Backward.tex <==
\subsection{Fourier Analysis of Motion Representations}
\label{subsec:forward_backward}
Fig.~\ref{fig:forward_backward_analysis} analyzes the signal spectra of the forward and backward motion representations (see Fig.~\ref{fig:forward_backward}). We take a vertical slice of pixels in Fig.~\ref{fig:forward_backward_analysis}~(a) as an example, and represent their forward or backward motion over 33 consecutive video frames as functions of time. At each vertical pixel location, we conduct 1-D Fourier transform of the motion signal along the temporal dimension. The results are visualized in Figs.~\ref{fig:forward_backward_analysis} (c) and (d) for the forward and backward representations, respectively. To ease comparison, we highlight the cut-off frequency in red. As shown, the backward motion representation tends to have more high-frequency components, being less smooth temporally. A side experiment replacing forward motion with backward motion in our MoTIF shows a 0.4dB PSNR loss on Gopro-\textit{average}. More results are provided in the supplementary document.  

%different motion representations, fast Fourier transform analyses to show that modeling backward motions as a function of time is more difficult than modeling forward motions. In Fig.~\ref{fig:forward_backward_analysis}, the ground-truth forward and backward motions of 33 temporally consecutive frames are used. We first analyze the time continuity of the ground-truth forward and backward motions. As shown in Fig.~\ref{fig:forward_backward_analysis} (c) and Fig.~\ref{fig:forward_backward_analysis} (d), forward motions (Fig.~\ref{fig:forward_backward_analysis} (c)) have smaller bandwidth than backward motions (Fig.~\ref{fig:forward_backward_analysis} (d)) for most of the pixels, implying that backward motions contain more high-frequency signals and thus it is more difficult to model as a function of time. We further analyze the spatailtemporal continuity of the ground-truth forward and backward motions in Fig.~\ref{fig:forward_backward_analysis} (e), Fig.~\ref{fig:forward_backward_analysis} (f), and Fig.~\ref{fig:forward_backward_analysis} (g). By applying 2-D fast Fourier transform, we observe that backward motions (orange) still contain more high-frequency signals than forward motions (blue) along both spatial and temporal axes. This means that backward motions are not only more difficult to model as a function of time $t$ but also a function of space $x,y$ and time $t$.


%We conduct a qualitative experiments to support our argument in Section~\ref{subsec:estimate_explicit_motion} that modeling backward motions as a function of time is more difficult than modeling forward motions. In Fig.~\ref{fig:forward_backward_analysis}, we use fast Fourier transform to analyze the ground-truth forward and backward motions of 33 temporally consecutive frames (Fig.~\ref{fig:forward_backward_analysis_a}). We first analyze the time continuity of the ground-truth forward and backward motions. As shown in Fig.~\ref{fig:forward_backward_analysis_c} and Fig.~\ref{fig:forward_backward_analysis_d}, forward motions have smaller bandwidth than backward motions for most of the pixels, meaning that backward motions contain more high-frequency signals and are more difficult to model than forward motions as a function of time. We further analyze the spatailtemporal continuity of the ground-truth forward and backward motions in Fig.~\ref{fig:forward_backward_analysis_e}, Fig.~\ref{fig:forward_backward_analysis_f}, and Fig.~\ref{fig:forward_backward_analysis_g}. By applying 2-D fast Fourier transform, we observe that backward motions still contain more high-frequency signals than forward motions along both spatial and temporal axes. Meaning that, backward motions are not only more difficult to model as a function of time $t$ but also a function of space $x,y$ and time $t$.

==> Chapter/4_experiment/Implementation_Details.tex <==
\subsection{Implementation Details}
\label{subsec:implementation_details}
We use Adam as our optimizer with $\beta_1=0.9$ and $\beta_2=0.999$ to end-to-end optimize our network. We use cosine annealing to decay our leaning rate from $10^{-4}$ to $10^{-7}$ every 150,000 iterations. To stably train our network, we use teacher forcing to replace our predicted motion with ground truth motion for a certain possibility, which will anneal from 1 to 0 in the first 150,000 iterations. The total number of iterations used to train our model is 600,000 with batch size 24. Following \cite{VideoINR}, we adopt a two-stage training manner. The space scale for the first 150,000 iterations is set to 4, while the next 450,000 iterations is uniformly chosen from $[1,4]$. In each batch, every input frame is down-sampled by the same space scale and cropped to $32 \times 32$. To predict the initial motion, if the size of the input frames is smaller than $128 \times 128$, the input frames will be first bilinear up-sampled to $128 \times 128$ due to the limitation of the motion estimator. We perform data augmentation by random rotating $90^{\circ}$, $180^{\circ}$ and $270^{\circ}$, and horizontal-flipping. We use Zooming SloMo\cite{ZSM} as our encoder and Raft-lite\cite{} as our motion estimator. The hyperparameter for forward warping $\alpha$ is set to $-20$ and the weight of the flow regularization loss $\beta$ is set to $0.01$.

==> Figures/forward_backward.tex <==
% \begin{figure}[t!]
%   \centering
%   \includegraphics[width=1.0\linewidth]{Figures/forward_backward.png}

%   \caption{Example of caption.}
%   \label{fig:forward_backward}
% \end{figure}
\begin{figure}[t!]
  \centering
  
  \begin{subfigure}[b]{0.45\linewidth}
  \includegraphics[trim={0 400 3814 0}
            ,clip,width=1.0\linewidth]{Figures/forward_backward.png}
    \caption{Forward Motion}
    \label{fig:forward_backward_a}
  \end{subfigure}
  \begin{subfigure}[b]{0.45\linewidth}
  \includegraphics[trim={3814 400 0 0}
            ,clip,width=1.0\linewidth]{Figures/forward_backward.png}
    \caption{Backward Motion}
    \label{fig:forward_backward_b}
  \end{subfigure}
  
  \caption{
  Illustration of forward and backward motion. Big yellow dots denote pixels accessible in the input video while small yellow dots refer to sub-pixels to be synthesized. The dash curves display the motion trajectories of pixels in the reference frame at $t=0$. The blue arrows are forward/backward motion in the form of displacement vectors. The red arrow shows the predicted forward displacement vector.
  }
  \vspace{-1.em}
  %\caption{
  %\textbf{An illustration of modeling forward motion and backward motion.}
  %The dash curves represent motion trajectories. The blue arrows represent the motions we can access to while the red arrow represents the predicted motion.
  %}
  \label{fig:forward_backward}
\end{figure}

==> Figures/forward_backward_analysis.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[b]{0.115\linewidth}
  \includegraphics[width=1.0\linewidth]{Figures/forward_backward_analysis/intensity.png}
    \caption{}
    \label{fig:forward_backward_analysis_a}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.115\linewidth}
  \includegraphics[width=1.0\linewidth]{Figures/forward_backward_analysis/motion.png}
    \caption{}
    \label{fig:forward_backward_analysis_b}
  \end{subfigure}
  \begin{subfigure}[b]{0.365\linewidth}
  \includegraphics[width=1.0\linewidth]{Figures/forward_backward_analysis/spec_for.png}
    \caption{}
    \label{fig:forward_backward_analysis_c}
  \end{subfigure}
  \begin{subfigure}[b]{0.365\linewidth}
  \includegraphics[width=1.0\linewidth]{Figures/forward_backward_analysis/spec_back.png}
    \caption{}
    \label{fig:forward_backward_analysis_d}
  \end{subfigure}
  % \begin{subfigure}[b]{0.32\linewidth}
  % \includegraphics[width=1.0\linewidth]{Figures/forward_backward_analysis/forward_3d.png}
  %   \caption{}
  %   \label{fig:forward_backward_analysis_e}
  % \end{subfigure}
  % \begin{subfigure}[b]{0.32\linewidth}
  % \includegraphics[width=1.0\linewidth]{Figures/forward_backward_analysis/backward_3d.png}
  %   \caption{}
  %   \label{fig:forward_backward_analysis_f}
  % \end{subfigure}
  % \begin{subfigure}[b]{0.32\linewidth}
  % \includegraphics[width=1.0\linewidth]{Figures/forward_backward_analysis/overlap_3d.png}
  %   \caption{}
  %   \label{fig:forward_backward_analysis_g}
  % \end{subfigure}
   \caption{Fourier analysis of forward and backward motion: (a) the slice of pixels whose forward/backward motion are analyzed, (b) the forward optical flow map, (c) the temporal signal spectra of forward motion, (d) the temporal signal spectra of backward motion. The red dots in (c)(d) highlight the cut-off frequencies.%, (e) the space-time signal spectrum of forward motion, (f) the space-time signal spectrum of backward motion, and (g) the superposition of (e) and (f). The red dots in (c)(d) highlight the cut-off frequencies.
  }
  \vspace{-1.0em}
   %\caption{We conduct an analysis over 33 consecutive video frames. (a) represents overlayed images we use. (b) visualizes the forward motion. The vertical red line indicates the pixels we sample to analyze. (c) and (d) are the spectrum of forward and backward motion with 1-D Fourier transform applied along the temporal dimension, respectively. The red dots indicates the cut-off frequency for each pixel. (e) and (f) are the 2-D spectrum of forward and backward motion with 2-D Fourier transform applied along both the spatial and temporal dimensions, respectively. (g) is the overlayed (e) and (f).}
  %\caption{We collect 33 temporally consecutive forward and backward optical flow maps, $\{M^H_{0\xrightarrow[]{}i}\}_{i=0}^{32}$ and $\{M^H_{i\xrightarrow[]{}0}\}_{i=0}^{32}$ and apply fast Fourier transform to ground-truth forward and backward motions respectively to analyze the temporal and spatial continuity of forward and backward motions. (a) is the overlayed $I^H_0$ and $I^H_{32}$. The red line indicates the pixels we sample to analyze. (b) is the visualization of $M^H_{0\xrightarrow[]{}32}$. The red line indicates the pixels we sample to analyze. (c) and (d) are the spectrum of forward and backward motions after 1-D fast Fourier transform over time, respectively. The red dots indicates the bandwidth for each pixel (e) is the 3-D spectrum of forward and backward motions after 2-D fast Fourier transform over time and y (the red line in (a) and (b)), respectively. (g) is the overlayed (e) and (f).}
  \label{fig:forward_backward_analysis}
\end{figure}


==> Figures/quantitative.tex <==
\setlength{\tabcolsep}{0.1pt}
\renewcommand{\arraystretch}{0.1}

\begin{figure*}[ht!]
    \centering
    \begin{tabular}{cc}
        %  TMNet~\cite{TMNet} &
        % \begin{tabular}{cccccccc}
        %     \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/TMNet/0_box.png}&
        %     \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/TMNet/1_box.png}&
        %     \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/TMNet/2_box.png}&
        %     \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/TMNet/3_box.png}&
        %     \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/TMNet/4_box.png}&
        %     \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/TMNet/5_box.png}&
        %     \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/TMNet/6_box.png}&
        %     \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/TMNet/7_box.png}
        %     \\
        %     \includegraphics[trim={2 214 722 174}
        %     ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/TMNet/0_box.png}&
        %     \includegraphics[trim={2 214 722 174}
        %     ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/TMNet/1_box.png}&
        %     \includegraphics[trim={2 214 722 174}
        %     ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/TMNet/2_box.png}&
        %     \includegraphics[trim={2 214 722 174}
        %     ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/TMNet/3_box.png}&
        %     \includegraphics[trim={2 214 722 174}
        %     ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/TMNet/4_box.png}&
        %     \includegraphics[trim={2 214 722 174}
        %     ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/TMNet/5_box.png}&
        %     \includegraphics[trim={2 214 722 174}
        %     ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/TMNet/6_box.png}&
        %     \includegraphics[trim={2 214 722 174}
        %     ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/TMNet/7_box.png}
        % \end{tabular}
        
        % \\ \\ \\
         VideoINR~\cite{VideoINR}  &
        \begin{tabular}{cccccccc}
            \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/VideoINR/0_box.png}&
            \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/VideoINR/1_box.png}&
            \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/VideoINR/2_box.png}&
            \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/VideoINR/3_box.png}&
            \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/VideoINR/4_box.png}&
            \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/VideoINR/5_box.png}&
            \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/VideoINR/6_box.png}&
            \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/VideoINR/7_box.png}
            \\
            \includegraphics[trim={2 214 722 174}
            ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/VideoINR/0_box.png}&
            \includegraphics[trim={2 214 722 174}
            ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/VideoINR/1_box.png}&
            \includegraphics[trim={2 214 722 174}
            ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/VideoINR/2_box.png}&
            \includegraphics[trim={2 214 722 174}
            ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/VideoINR/3_box.png}&
            \includegraphics[trim={2 214 722 174}
            ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/VideoINR/4_box.png}&
            \includegraphics[trim={2 214 722 174}
            ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/VideoINR/5_box.png}&
            \includegraphics[trim={2 214 722 174}
            ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/VideoINR/6_box.png}&
            \includegraphics[trim={2 214 722 174}
            ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/VideoINR/7_box.png}
        \end{tabular}
        \\ \\ \\
        \begin{tabular}{c}
         Ours 
        \\ \\ \\ \\ \\ \\ \\ \\ \\ \\
        \end{tabular}
        &
        \begin{tabular}{cccccccc}
            \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/Ours/0_box.png}&
            \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/Ours/1_box.png}&
            \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/Ours/2_box.png}&
            \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/Ours/3_box.png}&
            \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/Ours/4_box.png}&
            \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/Ours/5_box.png}&
            \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/Ours/6_box.png}&
            \includegraphics[width=0.105\linewidth]{Figures/quantitative/bmx/Ours/7_box.png}
            \\
            \includegraphics[trim={2 214 722 174}
            ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/Ours/0_box.png}&
            \includegraphics[trim={2 214 722 174}
            ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/Ours/1_box.png}&
            \includegraphics[trim={2 214 722 174}
            ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/Ours/2_box.png}&
            \includegraphics[trim={2 214 722 174}
            ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/Ours/3_box.png}&
            \includegraphics[trim={2 214 722 174}
            ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/Ours/4_box.png}&
            \includegraphics[trim={2 214 722 174}
            ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/Ours/5_box.png}&
            \includegraphics[trim={2 214 722 174}
            ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/Ours/6_box.png}&
            \includegraphics[trim={2 214 722 174}
            ,clip,width=0.105\linewidth]{Figures/quantitative/bmx/Ours/7_box.png}
        %\end{tabular}
        
        
        \\
        \\
        \\
        \\
        
        %&
        %\begin{tabular}{cccccccc}
        T=0&T=0.125&T=0.25&T=0.375&T=0.5&T=0.625&T=0.75&T=0.875
        \end{tabular}
        
        \\
        \\
        \\
        \\
        \\
        \\
        
        % TMNet~\cite{TMNet}  &
        % \begin{tabular}{cccccc}
        %     \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/TMNet/0_box.png}&
        %     \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/TMNet/1_box.png}&
        %     \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/TMNet/2_box.png}&
        %     \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/TMNet/3_box.png}&
        %     \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/TMNet/4_box.png}&
        %     \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/TMNet/5_box.png}
        %     \\
        %     \includegraphics[trim={302 302 152 2}
        %     ,clip,width=0.14\linewidth]{Figures/quantitative/motor/TMNet/0_box.png}&
        %     \includegraphics[trim={302 302 152 2}
        %     ,clip,width=0.14\linewidth]{Figures/quantitative/motor/TMNet/1_box.png}&
        %     \includegraphics[trim={302 302 152 2}
        %     ,clip,width=0.14\linewidth]{Figures/quantitative/motor/TMNet/2_box.png}&
        %     \includegraphics[trim={302 302 152 2}
        %     ,clip,width=0.14\linewidth]{Figures/quantitative/motor/TMNet/3_box.png}&
        %     \includegraphics[trim={302 302 152 2}
        %     ,clip,width=0.14\linewidth]{Figures/quantitative/motor/TMNet/4_box.png}&
        %     \includegraphics[trim={302 302 152 2}
        %     ,clip,width=0.14\linewidth]{Figures/quantitative/motor/TMNet/5_box.png}
        % \end{tabular}
        %\\ \\ \\
         VideoINR~\cite{VideoINR} &
        \begin{tabular}{cccccc}
            \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/VideoINR/0_box.png}&
            \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/VideoINR/1_box.png}&
            \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/VideoINR/2_box.png}&
            \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/VideoINR/3_box.png}&
            \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/VideoINR/4_box.png}&
            \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/VideoINR/5_box.png}
            \\
            \includegraphics[trim={302 302 152 2}
            ,clip,width=0.14\linewidth]{Figures/quantitative/motor/VideoINR/0_box.png}&
            \includegraphics[trim={302 302 152 2}
            ,clip,width=0.14\linewidth]{Figures/quantitative/motor/VideoINR/1_box.png}&
            \includegraphics[trim={302 302 152 2}
            ,clip,width=0.14\linewidth]{Figures/quantitative/motor/VideoINR/2_box.png}&
            \includegraphics[trim={302 302 152 2}
            ,clip,width=0.14\linewidth]{Figures/quantitative/motor/VideoINR/3_box.png}&
            \includegraphics[trim={302 302 152 2}
            ,clip,width=0.14\linewidth]{Figures/quantitative/motor/VideoINR/4_box.png}&
            \includegraphics[trim={302 302 152 2}
            ,clip,width=0.14\linewidth]{Figures/quantitative/motor/VideoINR/5_box.png}
        \end{tabular}
        \\ \\ \\
        \begin{tabular}{c}
         Ours 
        \\ \\ \\ \\ \\ \\ \\ \\ \\ \\
        \end{tabular}
        &
        \begin{tabular}{cccccc}
            \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/Ours/0_box.png}&
            \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/Ours/1_box.png}&
            \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/Ours/2_box.png}&
            \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/Ours/3_box.png}&
            \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/Ours/4_box.png}&
            \includegraphics[width=0.14\linewidth]{Figures/quantitative/motor/Ours/5_box.png}
            \\
            \includegraphics[trim={302 302 152 2}
            ,clip,width=0.14\linewidth]{Figures/quantitative/motor/Ours/0_box.png}&
            \includegraphics[trim={302 302 152 2}
            ,clip,width=0.14\linewidth]{Figures/quantitative/motor/Ours/1_box.png}&
            \includegraphics[trim={302 302 152 2}
            ,clip,width=0.14\linewidth]{Figures/quantitative/motor/Ours/2_box.png}&
            \includegraphics[trim={302 302 152 2}
            ,clip,width=0.14\linewidth]{Figures/quantitative/motor/Ours/3_box.png}&
            \includegraphics[trim={302 302 152 2}
            ,clip,width=0.14\linewidth]{Figures/quantitative/motor/Ours/4_box.png}&
            \includegraphics[trim={302 302 152 2}
            ,clip,width=0.14\linewidth]{Figures/quantitative/motor/Ours/5_box.png}
        %\end{tabular}
        \\
        \\
        \\
        \\
        %&
        %\begin{tabular}{cccccc}
        T=0 &T=0.17&T=0.33&T=0.50&T=0.67&T=0.83
        \end{tabular}
        \\
    \end{tabular}
    \caption{
        Subjective quality comparison. The temporal scaling factor of the upper example is 8 (in-distribution), whereas that of the lower example is 6 (out-of-distribution). Zoom in for better visualization.
    }
    %\vspace{-0.5em}
    \label{tbl:qualitative_results}
\end{figure*}
\renewcommand{\arraystretch}{1.}

==> Tables/ablation_forward_vs_backward.tex <==

\begin{table}[h]
    \centering
    \vspace{-0.15cm}
    %\caption{Forward vs. backward motion in our MoTIF following the x8 temporal scaling setting in Table 1. Metrics: PSNR/SSIM.}
    \caption{\textcolor{blue}{Forward~vs.~backward motion in MoTIF. Performance in PSNR/SSIM is reported under the difficult setting in Table 1: 8x temporal and 4x spatial scaling.}}
    \vspace{-0.25cm}
    \setlength{\tabcolsep}{2.0pt}
    \fontsize{8}{8}\selectfont
    \centering
    \begin{tabular}{c|c|c}
    \toprule
    %\hline
    &
    %Vid4 &
    %GoPro-\emph{Center} &
    GoPro-\emph{Average} &
    %Adobe-\emph{Center} &
    Adobe-\emph{Average}\\
    \midrule
    %\hline
    Backward &
    %- / - &
    %- / - &
    29.38 / 0.8693 &
    %- / - &
    29.14 / 0.8658 \\
    Forward &
    %\textbf{25.79} / \textbf{0.7745} &
    %\textbf{31.04} / \textbf{0.8877} &
    \textbf{30.04} / \textbf{0.8773} &
    %\textbf{30.63} / \textbf{0.8839} &
    \textbf{29.82} / \textbf{0.8750} \\
    \bottomrule
    %%\hline
    \end{tabular}
    \label{tab:forward v.s. backward}
    \vspace{-0.15cm}
\end{table}

==> Tables/ablation_study_flow_table4.tex <==
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.0}
\begin{table}
  \caption{Ablation experiment on tri-linear motion interpolation and multiple reference frames. Quality metrics: PSNR/SSIM.}
  %\caption{Ablation studies on flow. Forward Motions: Ours w/o reliability map}
  \fontsize{8}{8}\selectfont
  \centering
  \begin{tabular}{@{}c|cc@{}}
    \toprule
        Method &
        Gopro-\emph{Average} &
        %Gopro-\emph{Center} &
        Adobe-\emph{Average} 
        %Adobe-\emph{Center} 
        \\
    %\midrule
    %    Backward Motions &
    %    29.24 / 0.8672 &
    %    29.02 / 0.8641
    %    \\
    %    Forward Motions  &
    %    29.72 / 0.8714 &
    %    29.40 / 0.8669 &
    %    \\
    \midrule
        Tri-linear Motion &
        29.93 / 0.8759 &
        %30.89 / 0.8860 &
        29.64 / 0.8727 
        %30.42 / 0.8818
        \\
        Ours (2 ref) &
        30.08 / 0.8780 &
        %30.96 / 0.8868 &
        29.82 / 0.8750 
        %30.63 / 0.8839
        \\
        Ours (4 ref) &
        30.77 / 0.8948 &
        %31.44 / 0.9003 &
        30.37 / 0.8849 
        %31.03 / 0.8919
        \\
    \bottomrule
  \end{tabular}
  \label{tab:ablation_motion}
  \vspace{-1.em}
\end{table}
